uTNT: Unikernels for Efficient and Flexible Internet Probing

The last twenty years have seen the development and popularity of network measurement infrastructures. Internet measurement platforms have become common and have demonstrated their relevance in Internet understanding and security observation. However, despite their popularity, those platforms lack of flexibility and reactivity, as they are usually used for longitudinal measurements. As a consequence, they may miss detecting events that are security or Internet-related. During the same period, operating systems have evolved to virtual machines (VMs) as self-contained units for running applications, with the recent rise of unikernels, ultra-lightweight VMs tailored for specific applications, eliminating the need for a host OS. In this paper, we advocate that measurement infrastructures could take advantage of unikernels to become more flexible and efficient. We propose uTNT, a proof-of-concept unikernel-based implementation of TNT, a traceroute extension able to reveal MPLS tunnels. This paper documents the full toolchain for porting TNT into a unikernel and evaluates uTNT performance with respect to more traditional approaches. The paper also discusses a use case in which uTNT could find a suitable usage. uTNT source code is publicly available on Gitlab.

==> Bibliography.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                                   MISC                                        %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

@article{measurements_security,
author = "Safaei Pour, M. and Nader, C. and Friday, K. and Bou-Harb, E.",
title = "A Comprehensive Survey of Recent Internet Measurement Techniques for Cyber Security",
journal = "Computers \& Security",
volume = "128",
month = "May",
year = "2023",
}

@inproceedings{bgp_guided,
author = "Donnet, B.",
title = "Incentvies for {BGP} Guided {IP}-Level Topology Discovery",
booktitle = "Proc. Traffic and Measurement Analysis Workshop ({TMA})",
month = "May",
year = "2009",
}

@misc{openssl,
author = "{OpenSSL}",
title = "Cryptography and {SSL/TLS} Toolkit",
url = "https://www.openssl.org",
note = "[Last Accessed: October 24th, 2023]",
}

@misc{musl,
author = "{Felker, R. et al.}",
title = "musl",
url = "https://musl.libc.org",
note = "[Last Accessed: October 24th, 2023]",
}

@misc{kvm,
author = "{Red Hat.}",
title = "Kernel Virtual Machine",
url = "https://linux-kvm.org/page/Main_Page",
note = "[Last Accessed: October 24th, 2023]",
}

@misc{ovh_url,
author = "{OVH}",
title = "Global Cloud Service Provider | OVHcloud",
url = "https://us.ovhcloud.com",
note = "[Last Accessed: October 24th, 2023]",
}

@misc{protobuf,
author = "Google",
title = "Protocol Buffers",
url = "https://protobuf.dev",
note = "[Last Accessed: October 24th, 2023]",
}

@misc{memcached,
author = "{Danga Interactive}",
title = "memcached: A Distributed Memory Object Caching System",
url = "https://memcached.org",
note = "[Last Accessed: October 24th, 2023]",
}

@misc{nginx,
author = "{NGINX, Inc}",
title = "Advanced Load Balancer, Web Server, \& Reverse Proxy - NGINX",
url = "https://www.nginx.com",
note = "[Last Accessed: October 30th, 2023]",
}

@misc{sqlite,
author = "{D. Richard Hipp}",
title = "sqlite",
url = "https://sqlite.com",
note = "[Last Accessed: October 30th, 2023]",
}

@misc{solo5,
author = "{Williams, D. et al.}",
title = "Solo5: A Sandboxed Execution Environment",
url = "https://github.com/Solo5/solo5",
note = "[Last Accessed: October 24th, 2023]",
}

@misc{ukboot,
author = "Unikraft",
title = "ukboot: Unikraft bootstrapping",
url = "https://github.com/unikraft/unikraft/tree/staging/lib/ukboot",
note = "[Last Accessed: October 24th, 2023]",
}

@misc{lwip,
author = "{Dunkels, A. et al.}",
title = "lwip: Lightweith {IP}",
url = "https://savannah.nongnu.org/projects/lwip/",
note = "[Last Accessed: October 24th, 2023]",
}

@misc{cloc,
author = "{Al Danial}",
title = "cloc: Count Lines of Code",
url = "https://github.com/AlDanial/cloc",
note = "[Last Accessed: October 30th, 2023]",
}

@misc{url_ksm,
author = "Linux",
title = "Kernel Samepage Merging",
url = "https://docs.kernel.org/admin-guide/mm/ksm.html",
note = "[Last Accessed: October 24th, 2023]",
}

@misc{url_aws,
title = "AWS",
author = "Amazon",
howpublished = "https://aws.amazon.com",
note = "[Last Accessed: October 24th, 2023]"
}

@misc{url_google_cloud,
title = "Google Cloud Platform",
author = "Google",
howpublished = "https://cloud.google.com/",
note = "[Last Accessed: October 24th, 2023]"
}

@misc{url_dockerhub,
author = "Docker",
title = "DockerHub: Build and Ship any Application Anywhere",
url = "https://hub.docker.com",
note = "[Last Accessed: October 24th, 2023]",
}

@misc{url_vagrantcloud,
author = "Vagrant",
title = "Vagrant Cloud",
url = "https://app.vagrantup.com/boxes/search",
note = "[Last Accessed: October 24th, 2023]",
}

@article{outages,
author = "Aceto, G. and Botta, A. and Marchetta, P. and Persico, V. and Pescap\'e, A.",
title = "A Comprehensive Survey on {I}nternet Outages",
journal = "Journal of Network and Computer Applications",
volume = "113",
month = "July",
year = "2018",
pages = "36--63",
}

@misc{url_utnt,
author = "Gaulthier Gain",
title = "utnt",
url = "https://gitlab.uliege.be/Gaulthier.Gain/utnt",
note = "[Last Accessed: May 6th, 2024]",
}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                           scamper + TNT                                       %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
@TECHREPORT{traceroute,
author = "{V. Jacobson et al.}",
title = "traceroute",
institution = "{UNIX}",
type = "man page",
year = "1989",
note = "See source code: \url{ftp://ftp.ee.lbl.gov/traceroute.tar.gz}",
}

@ARTICLE{mpls-ccr,
author = "Donnet, B. and Luckie, M. and M\'erindol, P. and Pansiot, J.-J.",
title = "Revealing {MPLS} Tunnels Obscured from Traceroute",
journal = "{ACM} {SIGCOMM} Computer Communication Review",
year = "2012",
volume = "42",
number = "2",
month = "April",
pages = "87--93",
}

@INPROCEEDINGS{loadBalancing,
author = "Augustin, B. and Teixeira, R. and Friedman, T.",
title = "Measuring Load-Balanced Paths in the {I}nternet",
booktitle = "Proc. {ACM/USENIX} Internet Measurement Conference ({IMC})",
year = "2007",
month = "November",
}

@ARTICLE{alias,
author = "Keys, K.",
title = "{I}nternet-Scale {IP} Alias Resolution Techniques",
journal = "{ACM} {SIGCOMM} Computer Communication Review",
year = "2010",
volume = "40",
number = "1",
pages = "50--55",
month = "January",
}

@MISC{nanog,
author = "Gavron, E.",
title = "{NANOG} traceroute",
note = "See \url{http://man.he.net/man8/traceroute-nanog}",
}

@ARTICLE{survey,
author = "Donnet, B. and Friedman, T.",
title = "{I}nternet Topology Discovery: a Survey",
journal = "{IEEE} Communications Surveys and Tutorials",
year = "2007",
volume = "9",
number = "4",
month = "December",
}

@INPROCEEDINGS{fingerprinting,
author = "Vanaubel, Y. and Pansiot, J.-J. and M\'erindol, P. and Donnet, B.",
title = "Network Fingerprinting: {TTL}-Based Router Signature",
booktitle = "Proc. {ACM} Internet Measurement Conference ({IMC})",
year = "2013",
month = "October",
}

@INPROCEEDINGS{tnt-tma,
author = "Vanaubel, Y. and Luttringer, J.-R. and M\'erindol, P. and Pansiot, J.-J. and Donnet, B.",
title = "{TNT}, Watch me Explode: A Light in the Dark for Revealing {MPLS} Tunnels",
booktitle = "Proc. {IFIP} Network Traffic Measurement and Analysis Conference ({TMA})",
year = "2019",
month = "June",
}

@ARTICLE{tnt-tnsm,
author = "Luttringer, J.-R. and Vanaubel, Y. and M\'erindol, P. and Pansiot, J.-J. and Donnet, B.",
title = "Let There Be Light: Revealing Hidden {MPLS} Tunnels with {TNT}",
journal = "{IEEE} Transactions on Network and Service Management ({TNSM})",
year = "2020",
volume = "17",
number = "2",
pages = "1239--1253",
month = "June",
}

@INPROCEEDINGS{mpls-invisible,
author = "Vanaubel, Y. and M\'erindol, P. and Pansiot, J.-J. and Donnet, B.",
title  = "Through the Wormhole: Tracking Invisible {MPLS} Tunnels",
booktitle = "Proc. ACM Internet Measurement Conference ({IMC})",
year = "2017",
month = "November",
}

@INPROCEEDINGS{scamper,
author = "Luckie, M.",
title = "Scamper: a Scalable and Extensible Packet Prober for Active Measurement of the {I}nternet",
booktitle = "Proc. {ACM} Internet Measurement Conference ({IMC})",
year = "2010",
month = "November",
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                 Network Measurement Infrastructure                            %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
@INPROCEEDINGS{ark,
author = "claffy, {kc} and Hyun, Y. and Keys, K. and Fomenkov, M. and Krioukov, D.",
title = "{I}nternet Mapping: from Art to Science",
booktitle = "Proc. {IEEE} Cybersecurity Application and Technologies Conference for Homeland Security ({CATCH})",
year = "2009",
month = "March",
}

@INPROCEEDINGS{skitter,
author = "Huffaker, B. and Plummer, D. and Moore, D and claffy, {k}",
title = "Topology Discovery By Active Probing",
booktitle = "Proc. Symposium on Applications and the Internet ({SAINT})",
year = "2002",
month = "January",
}

@INPROCEEDINGS{neti,
author = "Simpson, C.R . and Riley, G. F.",
title = "{NETI}@home: A Distributed Approach to Collecting End-to-End Network Performance Measurements",
booktitle = "Proc. Passive and Active Measurement Workshop ({PAM})",
year = "2004",
month = "April",
}

@INPROCEEDINGS{dipzoom,
author = "Wen, Z. and Triukose, S. and Rabinovich, M.",
title = "Facilitating Focused Internet Measurements",
booktitle = "Proc. {ACM} {SIGMETRICS}",
year = "2007",
month = "June",
}

@INPROCEEDINGS{ntap,
author = "Masui, K. and Kadobayashi, Y.",
title = "{N-TAP}: A Platform of Large-Scale Distributed Measurement for Overlay Network Applications",
booktitle = "Proc. International Workshop on Dependable and Sustainable Peer-to-Peer Systems ({DAS-P2P})",
year = "2007",
month = "January",
}

@ARTICLE{dimes,
author = "Shavitt, Y. and Shir, E.",
title = "{DIMES}: Let the Internet Measure Itself",
journal = "{ACM} {SIGCOMM} Computer Communication Review",
volume = "35",
number = "5",
year = "2005",
}

@INPROCEEDINGS{scriptroute,
author = "Spring, N. and Wetherall, D. and Anderson, T.",
title = "Scriptroute: A Public {I}nternet Measurement Facility",
booktitle = "Proc. {USENIX} Symposium on Internet Technologies and Systems ({USITS})",
year = "2002",
month = "March",
note = "See \url{http://www.cs.washington.edu/research/networking/scriptroute/}"
}

@MISC{planetLab,
author = "{P}lanet{L}ab Consortium",
title = "{P}lanet{L}ab project",
note = "See \url{http://www.planet-lab.org}",
year = "2002",
}

@ARTICLE{ripe_lessons,
author = "Bajpai, V. and Eravuchira, S. J. and Schonwalder, J.",
title = "Lessons Learned from Using the {RIPE} {A}tlas Platform for Measurement Research",
journal = "{ACM} {SIGCOMM} Computer Communication Review",
year = "2015",
volume = "45",
number = "3",
pages = "35--42",
month = "July",
}

@ARTICLE{measurementPlatforms,
author = "Bajpai, V. and Schonwalder, J.",
title = "A Survey on {I}nternet Performance Measurement Platforms and Related Standardization Efforts",
journal = "{IEEE} Communications Surveys \& Tutorials",
year = "2015",
volume = "17",
number = "3",
pages = "1313--1341",
month = "April",
}

@MISC{ripe,
author = "{{RIPE} Network Coordination Center}",
title = "Atlas",
year = "2010",
note = "See \url{https://atlas.ripe.net}",
}

@INPROCEEDINGS{edgenet,
author = "Senel, B. C. and Mouchet, M. and Cappos, J. and Fourmaux, O. and Friedman, T. and McGeer, R.",
title = "{E}dge{N}et: A Multi-Tenant and Multi-Provider Edge Cloud",
booktitle = "Proc. International Workshop on Edge Systems, Analytics and Networking",
month = "April",
year = "2021",
}

@ARTICLE{dcart,
author = "M\'erindol, P. and David, P. and Pansiot, J.-J. and Clad, F. and Vissicchio, S.",
title = "A Fine-Grained Multi-Source Measurement Platform Correlating Routing Transitions with Packet Losses",
journal = "Computer Communication ({COMCOM})",
volume = "129",
year = "2018",
pages = "166--183",
month = "September",
}

@ARTICLE{mlab,
title = "M-Lab: User Initiated Internet Data for the Research Community",
author = "Gill, P. and Diot, C. and Ohlsen, L. Y. and Mathis, M. and Soltesz, S.",
journal = "{ACM} {SIGCOMM} Computer Communication Review",
number = "52",
volume = "1",
year = "2022",
month = "January",
}

@INPROCEEDINGS{iplane,
author = "Madhyastha, H. V. and Isdal, T. and Piatek, M. and Dixon, C. and Anderson, T. and Krishnamurthy, A. and Venkataramani, A.",
title = "i{P}lane: An Information Plane for Distributed Services",
booktitle = "Proc. {USENIX} Symposium on Operating Systems Design and Implementation ({OSDI})",
year = "2006",
month = "November",
}

@inproceedings {sybil,
author = "Cunha, I. and Marchetta, P. and Calder, M. and Chiu, Y. and Machado, B. and Pescap{\`e}, A. and Giotsas, V. and Madhyastha, H. and Katz-Bassett, E.",
title = "Sibyl: A Practical {I}nternet Route Oracle",
booktitle = "Proc. {USENIX} Symposium on Networked Systems Design and Implementation ({NSDI})",
year = "2016",
month = "March",
}

@ARTICLE{seti,
author = "Anderson, D.~P. and Cobb, J. and Korpela, E. and Lebofsky, M. and Werthimer, D.",
title = "{SETI}@home: An Experiment in Public-Resource Computing",
journal = "Communications of the {ACM}",
volume = "45",
number = "11",
year = "2002",
month = "November",
pages = "56--61",
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                                Dockers and VMs                                %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

@misc{docker-exploits,
title = "Docker Fixes Vulnerabilities, Shares Plans For Making Platform Safer",
author = "Kovacs, E.",
year = "2014",
howpublished = "\url{http://www.securityweek.com/docker-fixes-vulnerabilities-shares-plans-making-platform-safer}",
note = "[Last Accessed: October 26th, 2023]"
}

@misc{ncc-hardening,
title = "Understanding and Hardening Linux Containers",
author = {Grattafiori, A.},
year = "2016",
howpublished = "\url{https://research.nccgroup.com/2016/05/05/understanding-and-hardening-linux-containers/}",
note = "[Last Accessed: October 26th, 2023]"
}

@misc{docker_url,
title = "{Docker}",
author = "{Hykes, S. et al}",
year = "2018",
howpublished = "\url{https://docker.com/}",
note = "[Last Accessed: October 26th, 2023]"
}

@misc{lxc_url,
title = "{Linux Containers}",
author = "{Lezcano D., Hallyn S., Graber S.}",
year = "2008",
howpublished = "\url{https://linuxcontainers.org}",
note = "[Last Accessed: October 26th, 2023]"
}

@misc{libvirt_url,
title = "{Libvirt}",
author = "{Ubuntu}",
year = "n.d",
howpublished = "\url{https://ubuntu.com/server/docs/virtualization-libvirt}",
note = "[Last Accessed: October 26th, 2023]"
}

@inproceedings{ArcangeliKSM,
title = "Increasing memory density by using {KSM}",
author = "Arcangeli, A. and Eidus, I. and Wright, C.",
year = "2009",
booktitle = "Proc. Linux Symposium",
month = "January",
}

@inproceedings{NaiXiaUksm,
title = "{UKSM}: Swift Memory Deduplication via Hierarchical and Adaptive Memory Region Distilling",
author = "Xia, N. and Tian, C. and Luo, Y. and Liu, H. and Wang, X.",
year = "2018",
month = "February",
booktitle = "Proc. {USENIX} Conference on File and Storage Technologies ({FAST})",
}

@inproceedings{MillerKSMUI,
title= "{KSM++}: Using {I/O}-based hints to make memory-deduplication scanners more efficient",
author = "Miller, K. and Franz, F. and Groeninger, T. and Rittinghaus, M. and Hillenbrand, M. and Bellosa, F.",
year = "2012",
booktitle = "Proc. {ASPLOS} Workshop on Runtime Environments, Systems, Layering and Virtualized Environments ({RESoLVE})",
month = "March",
}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                                Unikernels                                     %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
@article{unikernel,
author = "Madhavapeddy, A. and Scott, D. J.",
title = "Unikernels: The Rise of the Virtual Library Operating Systems",
journal = "Communications of the {ACM}",
volume = "57",
number = "1",
month = "January",
year = "2014",
pages = "61--69",
}

@phdthesis{kantee,
author = "Kantee, A.",
title = "Flexible Operating Systems Internals: The Design and Implementation of the Anykernel and Rump Kernels",
school = "Aalto University",
year = "2012",
}

@inproceedings{clothing,
author = "Kuo, H.-C. and Williams, D. and Koller, R. and Mohan, S.",
title = "A {L}inux in Unikernel Clothing",
booktitle = "Proc. European Conference on Computer Systems ({EuroSys})",
month = "April",
year = "2020",
}

@inproceedings{jitsu,
author = "Madhavapeddy, A. and Leonard, T. and Skjegstad, M. and Gazagnaire, T. and Sheets, D. and Scott, D. and Mortier, R. and Chaudhry, A. and Singh, B. and Ludlam, J. and Crowcroft, J. and Leslie, I.",
title = "{J}itsu: Just-In-Time Summoning of Unikernels",
booktitle = "Proc. {USENIX} Sympositum on Networked Systems Design and Implementation ({NSDI})",
year = "2015",
month = "May",
}

@inproceedings{unikraft,
author = "Kuenzer, S. and Badoiu, V.-A. and Lefeuvre, H. and Santhanam, S. and Jung, A. and Gain, G. and Soldani, C. and Lupu, C. and Teodorescu, S. and Raducanu, C. and Banu, C. and Mathy, L. and Deaconescu, R. and Raiciu, C. and Huici, F.",
title = "{U}nikraft: Fast, Specialized Unikernels the Easy Way",
series = "In: Proc. European Conference on Computer Systems ({EuroSys})",
year = "2021",
month = "April",
}

@misc{unikraft_github,
title = "{unikraft}",
author = "{unikraft}",
year = "n.d",
howpublished = "\url{https://github.com/unikraft}",
note = "[Last Accessed: October 26th, 2023]"
}

@inproceedings{MirageOS,
author = "Kuenzer, S. and Badoiu, V.-A. and Lefeuvre, H. and Santhanam, S. and Jung, A. and Gain, G. and Soldani, C. and Lupu, C. and Teodorescu, S. and Raducanu, C. and Banu, C. and Mathy, L. and Deaconescu, R. and Raiciu, C. and Huici, F.",
title = "{U}nikraft: Fast, Specialized Unikernels the Easy Way",
booktite = "Proc. European Conference on Computer Systems ({EuroSys})",
year = "2021",
month = "April",
}

@inproceedings{Kivity2014,
title = "{OSv}--Optimizing the Operating System for Virtual Machines",
author = {Kivity, A. and Laor, D. and Costa, G. and Enberg, P. and Har'El, N. and Marti, D. and Zolotarov; V.},
year = "2014",
month = "June",
booktitle = "Proc. {USENIX} Annual Technical Conference",
}

@inproceedings{lefeuvre2023loupe,
title="Loupe: Driving the Development of {OS} Compatibility Layers",
author="Lefeuvre, H. and Gain, G. and Bădoiu, V.-A. and Dinca, D. and Schiller, V.-R. and Raiciu, C. and Huici, F. and Olivier, P.",
booktitle = "Proc. {ACM} Conference on Architectural Support for Programming Languages and Operating Systems ({ASPLOS})",
year="2024",
month = "May",
}

@misc{unikraft_tools,
title = "{Unikraft Tools}",
author = "Gain, G.",
year = "2019",
url = "https://github.com/gaulthiergain/tools",
note = "[Last Accessed: October 24th, 2023]",
}

@inproceedings{xen_barham_2003,
author = "Barham, P. and Dragovic, B. and Fraser, K. and Hand, S. and Harris, T. and Ho, A. and Neugebauer, R. and Pratt, I. and Warfield, A.",
title = "Xen and the Art of Virtualization",
year = "2003",
month = "October",
booktitle = "Proc. ACM symposium on Operating systems principles ({SOSP})",
}

@inproceedings{firecracker2020,
author = "Agache, A. and Brooker, M. and Iordache, A. and Liguori, A. and Neugebauer, R. and Piwonka, P. and Popa, D.-M",
title = "Firecracker: Lightweight Virtualization for Serverless Applications",
booktitle = "Proc. {USENIX} Symposium on Networked Systems Design and Implementation ({NSDI})",
year = "2020",
month = "February",
}

@inproceedings{gain_socc,
author = "Gain, G. and Soldani, C. and Huici, F. and Mathy, L.",
title = "Want More Unikernels? Inflate Them!",
year = "2022",
booktitle = "Proc. Symposium on Cloud Computing ({SoCC})",
month = "November",
}

@misc{nanos,
author = "{The Nanos developers}",
title = "Nanos",
url = "https://nanos.org",
note = "[Last Accessed: October 24th, 2023]",
}

@inproceedings{microkernel_perf,
author = "Du, D. and Hua, Z. and Xia, Y. and Zang, B. and Chen, H.",
title = "{Xpc}: Architectural Support for Secure and Efficient Cross Process Call",
booktitle = "Proc. {ACM/IEEE} Annual International Symposium on Computer Architecture ({ISCA})",
year = "2019",
month = "June",
}

@inproceedings{microkernel_perf2,
author = "Hartig, H. and Hohmuth, M. and Liedtke, J. and Schonberg, S. and Wolter, J.",
title = "The Performance of $\mu$-kernel-based Systems",
booktitle = "Proc. {ACM} Symposium on Operating Systems Principles ({SOSP})",
month = "October",
year = "1997",
}

@inproceedings{Jacobsen2015,
author = "Jacobsen, C. and Khole, M. and Spall, S. and Bauer, S. and Burtsev, A.",
title = "Lightweight Capability Domains: Towards Decomposing the Linux Kernel",
year = "2015",
booktitle = "Proc. Workshop on Programming Languages and Operating Systems ({PLOS}).",
month = "October",
}

@misc{linuxKernel,
title = "{The Linux Kernel Archives}",
author = "Linus Torvalds",
year = "2019",
url = "https://www.kernel.org",
note = "[Last Accessed: October 24th, 2023]",
}


==> ethical.tex <==
% !TEX root = ./paper.tex
\section*{Ethical Considerations} 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
In this paper, we did not harm the network with measurements. We
rather demonstrated the flexibility nature of \utnt over traditional
approaches. As such, we believe this paper does not raise any ethical
concerns. However, as for any probing tool, \utnt must be used with care to
avoid burdening the network with probes. However, this responsibility
falls to the ones deploying \utnt for their own purposes. This being
said, because \tnt is built upon \scamper, it comes with probing
limits facilities, such as the number of packets per second to be
sent.


==> related.tex <==
% !TEX root = ./paper.tex
\section{Related Work}\label{related}
%%%%%%%%%%%%%%%%%%%%%%

\subsection{Internet Probing}\label{related.probing}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
For more than twenty years now, Internet measurement platforms have
become common~\cite{measurementPlatforms}. Most of them have been
deployed by researchers and came with predefined measurement
capacities~\cite{skitter,ark,ripe,mlab,iplane}.  Measurements are
usually performed by platform owner and collected data set is often
made available to the research community.  Those platforms typically
rely on dedicated hardware, located in well known places or run by an
army of volunteers. In parallel to those academic platforms, several
measurement infrastructures~\cite{dimes,neti,dipzoom} have been
deployed following the SETI@home~\cite{seti} model.  That kind of
infrastructure come with the advantage of potentially increasing the
probing sources, but at the cost of development difficulties
(tools must support a varieties of hardware, operating systems, and
local configuration) and irregular data collection.  Further, several
consortiums~\cite{planetlab,edgenet,scriptroute} have also built
distributed platforms on which researchers can possibly deployed
their own network measurement experiences.

All those solutions require either dedicated hardware (e.g., RIPE
Atlas~\cite{ripe}, Archipelago~\cite{ark}, or even PlanetLab~\cite
{planetlab}), either an adaptation of tools to running operating
system and libraries (e.g., PlanetLab~\cite{planetlab} or Dimes~\cite
{dimes}).  More recent ones relies on Kubernetes and VM deployment
(e.g., EdgeNet~\cite{edgenet}). None of those solutions is flexible,
fastly deployable, and comes with a very low memory footprint.

\subsection{Unikernels}\label{related.unikernels}
%%%%%%%%%%%%%%%%%%%%%%%%

There exist plenty of related work showing that unikernels bring great
benefits and impressive performance compared to traditional VMs and
containers. \ed{GG: continue}
